Geometric-Based Nail Segmentation for Clinical Measurements

A robust segmentation method that can be used to perform measurements on toenails is presented. The proposed method is used as the first step in a clinical trial to objectively quantify the incidence of a particular pathology. For such an assessment, it is necessary to distinguish a nail, which locally appears to be similar to the skin. Many algorithms have been used, each of which leverages different aspects of toenail appearance. We used the Hough transform to locate the tip of the toe and estimate the nail location and size. Subsequently, we classified the super-pixels of the image based on their geometric and photometric information. Thereafter, the watershed transform delineated the border of the nail. The method was validated using a 348-image medical dataset, achieving an accuracy of 0.993 and an F-measure of 0.925. The proposed method is considerably robust across samples, with respect to factors such as nail shape, skin pigmentation, illumination conditions, and appearance of large regions affected by a medical condition

==> Figures/13-ToenailDetection_FiguraNormalization_v1.tex <==
\begin{figure*}[!ht]
\centering
    \begin{subfigure}[t]{0.4\textwidth}
            \centering
            \includegraphics[height=120pt]{images/normalization/img_original}
            \caption{Original photograph of a left foot on the template.}
            \label{fig:normalization:a}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.4\textwidth}
            \centering
            \includegraphics[height=120pt]{images/normalization/img_normalized}
            \caption{Normalized image obtained by preprocessing Fig.\ \ref{fig:normalization:a}.}
            \label{fig:normalization:b}
    \end{subfigure}
%\caption{Image normalization using the template corners to perform an holography.}
%\label{fig:normalization}
\end{figure*}

==> Tables/14-Results_TableDatasets.tex <==
\begin{table}[]
    \centering
    \caption{Number of images in our datasets.}
    \begin{tabular}{@{}cc@{}}
    \toprule
    Dataset   & \begin{tabular}[c]{@{}c@{}}Number of\\ images\end{tabular} & n. nail regions & n. skin regions \\ \midrule
    Train & 257     &       6568 & 41413                                              \\
    Test  & 91      &       2309 & 15183                       \\ \bottomrule
    \end{tabular}
    \label{tab:datasets}
\end{table}

==> sections/00-Conflicts.tex <==
{\onecolumn
    \pagestyle{empty}
    \pagenumbering{gobble}
    
    \begin{center}
    \textbf{\LARGE Conflict of interest}\\ 
    \textsc{\Large Robust toenail detection}
    \end{center} \vspace*{1cm}
    
\noindent The  authors  whose  names  are  listed  immediately  below  certify  that  they  have  NO  affiliations  with  or  involvement  in  any organization or entity with any financial interest (such as honoraria; educational grants; participation in speakers’ bureaus;  membership, employment, consultancies, stock ownership, or other equity interest; and expert testimony or patent-licensing arrangements), or non financial interest (such as personal or professional relationships, affiliations, knowledge or beliefs) in
the subject matter or materials discussed in this manuscript.
\\[12pt]
\noindent \textbf{Author names:}

    \noindent Dr. Gabriel Moyà-Alcover \\
    Mr. Bernat Galmés \\
    Dr. Pedro Bibiloni \\
    Dr. Javier Varona \\
    Dr. Antoni Jaume-i-Capó
    

\vspace{0.3cm}
\noindent This statement is signed by all the authors to indicate agreement that the above information is true and correct: \vspace{0.5cm}

\noindent \textbf{Author's name} \hspace{3.0cm}  \textbf{Author's signature} \hspace{2.5cm}       \textbf{Date}  \\

\vspace*{1cm}
\noindent Dr. Gabriel Moyà-Alcover  \\
\\[12pt]
Mr. Bernat Galmés \\
\\[12pt]
Dr. Pedro Bibiloni \\
\\[12pt]
Dr. Javier Varona \\
\\[12pt]
Dr. Antoni Jaume-i-Capó

}

\newpage
\pagenumbering{arabic}


==> sections/00-CoverLetter.tex <==
{\onecolumn
    \pagestyle{empty}
    \pagenumbering{gobble}
    
    \begin{center}
    \textbf{\LARGE Cover letter of the manuscript}\\ 
    \textsc{\Large Robust toenail detection}
    \end{center} \vspace*{1cm}
    
    
    \noindent
    Dear Mr Editor % TODO: posar nom editor,
    
    \vspace{0.3cm}\noindent
    The attached manuscript \textit{Geometric-Based nail Segmentation for Clinical Measurements}, is submitted for publication as a full article to Multimedia Tools and Applications. We highlight that this manuscript is the authors' original work and has not been published nor has it been submitted elsewhere.
    
    \vspace{0.3cm}\noindent
    It is coauthored by
    Dr. Gabriel Moya-Alcover (corresponding author, gabriel.moya@uib.es);
    Mr. Bernat Galmés, Dr. Pedro Bibiloni, Dr. Javier Varona and Dr. Antoni Jaume-i-Capó from the University of the Balearic Islands.
    
    
    \vspace{0.3cm}\noindent
    
    
    
    \vspace{0.3cm}\noindent
    We would appreciate that you consider reviewing this manuscript.
    
    \vspace{0.3cm}\noindent
    Sincerely,
    
    \vspace{0.9cm}\noindent
    The authors. 
  
}

\newpage
\pagenumbering{arabic}


==> sections/00-Highlights.tex <==
{\onecolumn
    \pagestyle{empty}
    \pagenumbering{gobble}

    \begin{center}
    \textbf{\LARGE Highlights of the manuscript}\\ 
    \textsc{\Large ``Robust Toenail Detection''}
    \end{center} \vspace*{1cm}
    
    {
    \large
    \begin{itemize}[label={$\blacktriangleright$}]
    % Aquesta linea te exactament 85 caracters més els 6 de '\item' %%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item We introduce a method to segment
the  nail  of  big  toes  in  photographs  captured with a template specially designed for this task.
        \item We segment toenails by combining several algorithms, based on geometric and photometric features, each of them refining the previous result.
    \item The method has  been  validated  with  a  348-image clinical dataset.
    \item Several  performance measures are employed to quantify the ability of the method to discriminate nail and toe pixels. It achieves an accuracy of 0.993 and an  F-measure  of  0.92.
    \end{itemize}
    }
}

\newpage
\pagenumbering{arabic}


==> sections/02-Titlepage.tex <==
\newgeometry{
    top=35mm,
    bottom=30mm,
    outer=30mm,
    inner=30mm,
}
\begin{titlepage}
\begin{center}


\textsc{\LARGE Universitat de les Illes Balears}\\[1.5cm]

\textsc{\Large ~}\\[-0.5cm]

% Title
\HRule
{ \huge \bfseries Title \\[0.4cm] }

\HRule \\[1.1cm]

% Author and supervisor
\begin{minipage}{0.4\textwidth}
\begin{flushleft}
\emph{Author:}\\
Pedro Bibiloni Serrano
\end{flushleft}
\end{minipage}
~
\begin{minipage}{0.4\textwidth}
\begin{flushright}
\emph{Advisor:}\\
~
\end{flushright}
\end{minipage}

\vfill

% Bottom of the page
{\large January 1, 1970} \\[1cm]
\end{center}

\begin{flushright}

 
 



{\fontsize{10pt}{10pt}
\emph{
Disclaimer here.\\ 
~\\
The report may be freely copied and distributed provided the source is explicitly acknowledged.}
}
\end{flushright}

\end{titlepage}
\restoregeometry

==> sections/91-License.tex <==
\section*{License}

\copyright 2016. This 
%
preprint    % before peer-review process
            % or
%accepted    % just after acception, without journal formatting (embargo period?)
%
manuscript version is made available for personal use, internal institutional use and scholarly sharing purposes under the CC-BY-NC-ND 4.0 license (\url{http://creativecommons.org/licenses/by-nc-nd/4.0/}).

%The version of record has been published and assigned the following Digital Identifier Object:  \doi{10.1016/j.patcog.2016.07.023}.



==> sections/99-Examples.tex <==
\section{Examples: code usage}


This section contains several exemples of code usage, covering hyperlinks, footnotes, figures, code formatting, etc.
The rest of the document contains dummy text.


\begin{figure}[!ht]
\centering
\includegraphics[width=0.25\textwidth]{images/picture.png}
\caption{Diagrama funcional d'un sistema}
\label{diagrama-funcional}
\end{figure}

% Imatge no flotant
\begin{center}
\includegraphics[scale=0.4]{images/picture.png} \\ \nopagebreak[4]
Figura 1: Diagrama funcional d'un sistema
\end{center}



\begin{figure}
\centering
        \begin{subfigure}[t]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/picture.png}
                \caption{Diagrama 1 - Disseny}
                \label{diagrama-1}
        \end{subfigure}%
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[t]{0.3\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/picture.png}
                \caption{Diagrama 2 - Característiques}
                \label{diagrama-2}
        \end{subfigure}
\caption{Figura múltiple: diagrames relacionats}
\label{diagrames-1-2}
\end{figure}



\begin{lstlisting}
...
\end{lstlisting}



Nota a pie de página\footnote{\href{http://url.com/documento.pdf}{Click aqui}, para encontrar el documento.}.

Referencia bibliográfica en \citep{kass1988snakes}. Si no se pone ninguna cita, la entrada bibliográfica no aparecerá entre la bibliografía.

